First Sagittarius A* Event Horizon Telescope Results. V. Testing Astrophysical Models of the Galactic Center Black Hole

In this paper, we provide a first physical interpretation for the Event Horizon Telescope (EHT)'s 2017 observations of Sgr A*. Our main approach is to compare resolved EHT data at 230 GHz and unresolved non-EHT observations from radio to X-ray wavelengths to predictions from a library of models based on time-dependent general relativistic magnetohydrodynamics (GRMHD) simulations, including aligned, tilted, and stellar wind-fed simulations; radiative transfer is performed assuming both thermal and non-thermal electron distribution functions. We test the models against 11 constraints drawn from EHT 230 GHz data and observations at 86 GHz, 2.2 $\mu$m, and in the X-ray. All models fail at least one constraint. Light curve variability provides a particularly severe constraint, failing nearly all strongly magnetized (MAD) models and a large fraction of weakly magnetized (SANE) models. A number of models fail only the variability constraints. We identify a promising cluster of these models, which are MAD and have inclination $i \le$ 30$^\circ$. They have accretion rate $(5.2$-$9.5)\times10^{-9}M_\odot$yr$^{-1}$, bolometric luminosity $(6.8$--$9.2)\times10^{35}$ erg s$^{-1}$, and outflow power $(1.3$--$4.8)\times10^{38}$ erg s$^{-1}$. We also find that: all models with $i \ge$ 70$^\circ$ fail at least two constraints, as do all models with equal ion and electron temperature; exploratory, non-thermal model sets tend to have higher 2.2 $\mu$m flux density; the population of cold electrons is limited by X-ray constraints due to the risk of bremsstrahlung overproduction. Finally we discuss physical and numerical limitations of the models, highlighting the possible importance of kinetic effects and duration of the simulations.

==> Tables/BHAC_varkappa_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|ccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Frankfurt Variable $\kappa$ Models}
\label{tab:VKbhacPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 2.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-6}$ & 5.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.8$\times10^{-6}$ & 6.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.3$\times10^{-6}$ & 7.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.2$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 2.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-6}$ & 5.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-6}$ & 6.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-6}$ & 7.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.3$\times10^{-8}$ & 2.0$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 2.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-6}$ & 4.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-6}$ & 5.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.3$\times10^{-6}$ & 7.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &8.9$\times10^{-8}$ & 1.9$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-6}$ & 4.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-6}$ & 5.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.3$\times10^{-6}$ & 7.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.4$\times10^{-8}$ & 1.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-6}$ & 4.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-6}$ & 5.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-6}$ & 7.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-8}$ & 3.6$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.0$\times10^{-6}$ & 2.5$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.8$\times10^{-6}$ & 3.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.8$\times10^{-6}$ & 3.6$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-8}$ & 3.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.1$\times10^{-6}$ & 2.5$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.0$\times10^{-6}$ & 3.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.1$\times10^{-6}$ & 3.8$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-6}$ & 2.4$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.8$\times10^{-6}$ & 2.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.8$\times10^{-6}$ & 3.6$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &5.6$\times10^{-8}$ & 3.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-6}$ & 2.4$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.9$\times10^{-6}$ & 3.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.0$\times10^{-6}$ & 3.7$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.1$\times10^{-6}$ & 2.5$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.1$\times10^{-6}$ & 3.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.4$\times10^{-6}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.4$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.5$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-6}$ & 8.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 80.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.6$\times10^{-6}$ & 1.1$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-6}$ & 1.4$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.2$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-6}$ & 8.0$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 80.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &4.4$\times10^{-6}$ & 1.0$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-6}$ & 1.3$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 8.1$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.5$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-6}$ & 8.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.4$\times10^{-6}$ & 1.0$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-6}$ & 1.3$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.5$\times10^{-8}$ & 8.1$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.6$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 8.6$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.2$\times10^{-6}$ & 1.5$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 8.0$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 2.7$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-6}$ & 8.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.0$\times10^{-6}$ & 1.2$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 160.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.5$\times10^{-6}$ & 1.5$\times10^{37}$ & 4.5$\times10^{-4}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-8}$ & 4.4$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.8$\times10^{-7}$ & 6.1$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &7.7$\times10^{-7}$ & 1.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.1$\times10^{-6}$ & 2.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.5$\times10^{-6}$ & 3.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 4.3$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.7$\times10^{-7}$ & 5.9$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &7.5$\times10^{-7}$ & 1.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.1$\times10^{-6}$ & 2.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.5$\times10^{-6}$ & 3.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 4.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 5.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 40.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.4$\times10^{-7}$ & 1.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-6}$ & 3.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.9$\times10^{-8}$ & 4.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 5.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 40.0 & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-7}$ & 1.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 80.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 3.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.9$\times10^{-8}$ & 4.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 5.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.9$\times10^{-7}$ & 1.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 80.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 2.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.3$\times10^{-9}$ & 4.4$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &6.1$\times10^{-7}$ & 3.7$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 80.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.9$\times10^{-7}$ & 4.8$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-6}$ & 6.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.2$\times10^{-9}$ & 4.3$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 10.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.1$\times10^{-7}$ & 6.7$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.0$\times10^{-7}$ & 4.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &8.8$\times10^{-7}$ & 5.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 160.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.1$\times10^{-6}$ & 6.8$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.9$\times10^{-9}$ & 4.2$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.7$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-7}$ & 4.6$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 6.1$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.3$\times10^{-6}$ & 7.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.8$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.2$\times10^{-7}$ & 7.2$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-7}$ & 4.6$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 6.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.6$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.8$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.2$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-7}$ & 4.5$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-6}$ & 6.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.7$\times10^{37}$ & 1.2$\times10^{-2}$\\
M & -0.94 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.3$\times10^{-8}$ & 4.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 2.0$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 2.6$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-7}$ & 3.7$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.2$\times10^{-8}$ & 4.0$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.9$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 2.6$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-7}$ & 3.6$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.0$\times10^{-8}$ & 3.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-7}$ & 1.0$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-7}$ & 1.7$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-7}$ & 2.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 3.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 3.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.7$\times10^{-8}$ & 9.2$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.6$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 2.9$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-8}$ & 3.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.2$\times10^{-8}$ & 8.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.5$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 2.0$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.0$\times10^{-7}$ & 2.9$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 9.2$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-7}$ & 3.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-7}$ & 5.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-7}$ & 7.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &4.2$\times10^{-7}$ & 9.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 8.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 3.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.2$\times10^{-7}$ & 5.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-7}$ & 6.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.0$\times10^{-7}$ & 9.6$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.6$\times10^{-8}$ & 8.5$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.8$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.1$\times10^{-7}$ & 4.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 6.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-7}$ & 8.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.4$\times10^{-8}$ & 8.0$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 2.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-7}$ & 4.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-7}$ & 5.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-7}$ & 8.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.3$\times10^{-8}$ & 7.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-7}$ & 4.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-7}$ & 5.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-7}$ & 8.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & 0.0 & 10.0 & 1.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.9$\times10^{-8}$ & 5.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 9.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.1$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 1.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.6$\times10^{-8}$ & 5.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.8$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.1$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.1$\times10^{-8}$ & 5.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.0$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 1.3$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.6$\times10^{-8}$ & 4.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 9.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-8}$ & 1.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-8}$ & 4.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 7.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 80.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 9.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-8}$ & 1.3$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.8$\times10^{-8}$ & 3.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.2$\times10^{-8}$ & 6.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass &1.1$\times10^{-7}$ & 8.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass &1.4$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-8}$ & 1.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.6$\times10^{-8}$ & 3.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.9$\times10^{-8}$ & 6.5$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 80.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.0$\times10^{-7}$ & 8.5$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass &1.4$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.5$\times10^{-8}$ & 1.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.4$\times10^{-8}$ & 3.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.6$\times10^{-8}$ & 6.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.9$\times10^{-8}$ & 8.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-8}$ & 1.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &4.1$\times10^{-8}$ & 3.4$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.3$\times10^{-8}$ & 6.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.6$\times10^{-8}$ & 7.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-8}$ & 1.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.1$\times10^{-8}$ & 5.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.5$\times10^{-8}$ & 7.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.94 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.5$\times10^{-9}$ & 4.1$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.1$\times10^{-8}$ & 2.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &5.3$\times10^{-8}$ & 2.6$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &7.1$\times10^{-8}$ & 3.4$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.4$\times10^{-9}$ & 4.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.0$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &5.3$\times10^{-8}$ & 2.5$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.0$\times10^{-8}$ & 3.4$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.2$\times10^{-9}$ & 3.9$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &3.9$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &5.2$\times10^{-8}$ & 2.5$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.9$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.0$\times10^{-9}$ & 3.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.1$\times10^{-8}$ & 1.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.2$\times10^{-8}$ & 2.5$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.0$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-9}$ & 3.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.1$\times10^{-8}$ & 10.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 80.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-8}$ & 2.5$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 3.5$\times10^{38}$ & 9.3$\times10^{-1}$\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Critical_Beta_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{ccc|ccc|c|cccccc|c|c|c}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Critical Beta Models}
\label{tab:betacritPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
}
\startdata
S & -0.94 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail\\
S & -0.94 & 50.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
S & -0.94 & 90.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.5 & 10.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
S & -0.5 & 50.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
S & -0.5 & 90.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
S & 0.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
S & 0.0 & 50.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail\\
S & 0.0 & 90.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
S & 0.5 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail\\
S & 0.5 & 50.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
S & 0.5 & 90.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Pass\\
S & 0.94 & 10.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
S & 0.94 & 50.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
S & 0.94 & 90.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.94 & 50.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.94 & 90.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass\\
M & -0.5 & 50.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 90.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.0 & 50.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail\\
M & 0.0 & 90.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.5 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail\\
M & 0.5 & 50.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 90.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
M & 0.94 & 50.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 90.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Frankfurt_All_Epsilon_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{ccccc|ccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Frankfurt Fixed $\kappa$, Variable Efficiency Models}
\label{tab:frankfurtfkPF}
\tablehead{ \colhead{$\epsilon$}  &  %
\colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
0.05 & S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.0$\times10^{-8}$ & 2.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-7}$ & 6.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.7$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.9$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 6.2$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.3$\times10^{-7}$ & 2.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-6}$ & 3.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.7$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.9$\times10^{-7}$ & 6.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.4$\times10^{-7}$ & 2.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-6}$ & 3.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.8$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.9$\times10^{-7}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.6$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-7}$ & 7.0$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 3.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-8}$ & 3.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-6}$ & 3.5$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.0$\times10^{-6}$ & 3.7$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-6}$ & 2.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-6}$ & 3.5$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-6}$ & 2.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-6}$ & 3.6$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.4$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & -0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.1$\times10^{-6}$ & 3.8$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.05 & S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 9.0$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-6}$ & 6.8$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.7$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.1$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-6}$ & 6.7$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.5$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-6}$ & 6.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.6$\times10^{-8}$ & 8.4$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-6}$ & 7.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.2$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-6}$ & 3.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.0 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-6}$ & 7.5$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.05 & S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-7}$ & 3.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-6}$ & 4.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.1$\times10^{-6}$ & 8.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.1$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.2$\times10^{-6}$ & 4.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.2$\times10^{-6}$ & 9.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.5$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 50.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.1$\times10^{-6}$ & 4.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.9$\times10^{-6}$ & 8.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.0$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 4.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-6}$ & 8.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.1$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-7}$ & 3.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-6}$ & 8.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail &6.3$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.05 & S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.3$\times10^{-9}$ & 4.4$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 10.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass &1.1$\times10^{-7}$ & 6.6$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-7}$ & 3.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.7$\times10^{-7}$ & 5.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.1$\times10^{-9}$ & 4.2$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 30.0 & 10.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-7}$ & 6.5$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.4$\times10^{-7}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-6}$ & 6.6$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.8$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.4$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.2$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-6}$ & 7.7$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &7.2$\times10^{-7}$ & 4.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.2$\times10^{-7}$ & 7.1$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &7.1$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.05 & M & -0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 5.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.8$\times10^{-8}$ & 8.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 1.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 5.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.4$\times10^{-8}$ & 8.0$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 1.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-8}$ & 4.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.8$\times10^{-8}$ & 7.4$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-8}$ & 4.4$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.3$\times10^{-8}$ & 6.9$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.5$\times10^{-8}$ & 4.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-8}$ & 6.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.05 & M & -0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 9.1$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 3.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-7}$ & 5.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &3.8$\times10^{-7}$ & 9.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.8$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 2.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-7}$ & 4.8$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-7}$ & 8.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.4$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 2.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-7}$ & 4.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-7}$ & 8.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 8.0$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 4.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-8}$ & 7.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 3.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & -0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.05 & M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.2$\times10^{-8}$ & 5.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 8.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.1$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.9$\times10^{-8}$ & 4.9$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.0$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.6$\times10^{-8}$ & 4.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.2$\times10^{-8}$ & 4.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.9$\times10^{-8}$ & 4.2$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.0 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.05 & M & 0.5 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 10.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.2$\times10^{-7}$ & 2.7$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 3.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-7}$ & 8.4$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.1$\times10^{-7}$ & 2.6$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.6$\times10^{-8}$ & 3.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.4$\times10^{-8}$ & 7.7$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.5$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.9$\times10^{-7}$ & 2.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.4$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.4$\times10^{-8}$ & 6.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.0$\times10^{-8}$ & 6.5$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.5$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.05 & M & 0.94 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.5$\times10^{-9}$ & 4.1$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.9$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.6$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.4$\times10^{-9}$ & 4.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.2$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.8$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.6$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.2$\times10^{-9}$ & 3.9$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &2.1$\times10^{-8}$ & 1.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.5$\times10^{-8}$ & 3.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &8.0$\times10^{-9}$ & 3.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.0$\times10^{-8}$ & 9.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.7$\times10^{-9}$ & 3.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.0$\times10^{-8}$ & 9.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.05 & M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &6.8$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.0$\times10^{-8}$ & 2.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-7}$ & 6.2$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.8$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-6}$ & 3.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.9$\times10^{-9}$ & 2.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 6.1$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.3$\times10^{-7}$ & 2.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.7$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 6.2$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.5$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.8$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.0$\times10^{-7}$ & 6.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.9$\times10^{-7}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 3.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.6$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 3.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-8}$ & 3.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-6}$ & 3.6$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 30.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.2$\times10^{-6}$ & 3.8$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 9.9$\times10^{36}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-6}$ & 2.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-6}$ & 3.7$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.1$\times10^{-6}$ & 3.7$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.4$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & -0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.2$\times10^{-6}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.10 & S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 9.0$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.0$\times10^{-6}$ & 6.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.7$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-6}$ & 6.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.5$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.0$\times10^{-6}$ & 7.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.6$\times10^{-8}$ & 8.4$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-6}$ & 7.5$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.2$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.0 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-6}$ & 7.7$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.10 & S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-7}$ & 3.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-6}$ & 4.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.1$\times10^{-6}$ & 8.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.2$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.2$\times10^{-6}$ & 4.7$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.2$\times10^{-6}$ & 9.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.6$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 4.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.9$\times10^{-6}$ & 8.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.1$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-6}$ & 8.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.1$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-7}$ & 3.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-6}$ & 8.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.10 & S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.3$\times10^{-9}$ & 4.4$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-7}$ & 6.6$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-7}$ & 3.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.9$\times10^{-7}$ & 6.0$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.1$\times10^{-9}$ & 4.3$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-7}$ & 6.5$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.4$\times10^{-7}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-6}$ & 6.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.8$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.4$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.2$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.3$\times10^{-6}$ & 8.0$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &7.2$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.5$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.2$\times10^{-7}$ & 7.1$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &7.1$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.5$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.10 & M & -0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 5.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.8$\times10^{-8}$ & 8.4$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 5.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.5$\times10^{-8}$ & 8.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 1.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-8}$ & 4.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.9$\times10^{-8}$ & 7.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-8}$ & 4.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.3$\times10^{-8}$ & 7.0$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.5$\times10^{-8}$ & 4.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-8}$ & 6.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.10 & M & -0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 9.2$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 3.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-7}$ & 5.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &3.8$\times10^{-7}$ & 9.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 8.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 2.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-7}$ & 4.8$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-7}$ & 8.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.5$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 2.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-7}$ & 4.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-7}$ & 8.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 8.0$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 4.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-8}$ & 7.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 4.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & -0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.10 & M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.3$\times10^{-8}$ & 5.2$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 8.8$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.1$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.0$\times10^{-8}$ & 4.9$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.1$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.6$\times10^{-8}$ & 4.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.2$\times10^{-8}$ & 4.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.9$\times10^{-8}$ & 4.2$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.0 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.10 & M & 0.5 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.7$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 10.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-7}$ & 2.7$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-7}$ & 8.4$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.1$\times10^{-7}$ & 2.6$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.6$\times10^{-8}$ & 3.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.4$\times10^{-8}$ & 7.7$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.5$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.9$\times10^{-7}$ & 2.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.4$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.5$\times10^{-8}$ & 7.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.0$\times10^{-8}$ & 6.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.5$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.10 & M & 0.94 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.5$\times10^{-9}$ & 4.1$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.9$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.7$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.4$\times10^{-9}$ & 4.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.8$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.7$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.2$\times10^{-9}$ & 3.9$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.6$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &8.0$\times10^{-9}$ & 3.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.1$\times10^{-8}$ & 9.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.6$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.7$\times10^{-9}$ & 3.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.0$\times10^{-8}$ & 9.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.10 & M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &6.8$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.0$\times10^{-8}$ & 2.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 6.1$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.8$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 4.4$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.9$\times10^{-9}$ & 2.2$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 5.9$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.4$\times10^{-7}$ & 2.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 4.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.7$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 6.0$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.6$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 4.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.8$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.9$\times10^{-7}$ & 6.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &10.0$\times10^{-7}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.6$\times10^{-9}$ & 2.1$\times10^{35}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.0$\times10^{-7}$ & 6.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-8}$ & 3.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-6}$ & 1.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.3$\times10^{-6}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-6}$ & 9.9$\times10^{36}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-6}$ & 2.4$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 30.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-6}$ & 4.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-6}$ & 9.6$\times10^{36}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.3$\times10^{-6}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 9.7$\times10^{36}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.3$\times10^{-6}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.4$\times10^{-8}$ & 3.4$\times10^{35}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-6}$ & 9.7$\times10^{36}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & -0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.4$\times10^{-6}$ & 4.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
0.20 & S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 9.0$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.2$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-6}$ & 7.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.8$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-7}$ & 1.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 30.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-6}$ & 7.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.6$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-6}$ & 7.4$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.6$\times10^{-8}$ & 8.5$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-6}$ & 7.7$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.3$\times10^{34}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-7}$ & 1.1$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-6}$ & 3.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.0 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-6}$ & 7.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
0.20 & S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-7}$ & 3.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.2$\times10^{-6}$ & 4.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.1$\times10^{-6}$ & 8.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.4$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.2$\times10^{-6}$ & 4.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &4.2$\times10^{-6}$ & 9.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 30.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.7$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 4.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.9$\times10^{-6}$ & 8.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.6$\times10^{-7}$ & 3.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-6}$ & 4.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-6}$ & 8.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-6}$ & 1.3$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-7}$ & 3.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 4.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-6}$ & 8.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.5 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-6}$ & 1.4$\times10^{38}$ & 4.2$\times10^{-3}$\\
0.20 & S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.3$\times10^{-9}$ & 4.4$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-7}$ & 6.6$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-7}$ & 3.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.0$\times10^{-6}$ & 6.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.1$\times10^{-9}$ & 4.3$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.1$\times10^{-7}$ & 6.5$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.5$\times10^{-7}$ & 3.9$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-6}$ & 7.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.8$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.4$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &7.2$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.4$\times10^{-6}$ & 8.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-7}$ & 4.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-6}$ & 8.8$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.2$\times10^{-7}$ & 7.1$\times10^{36}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.0$\times10^{-7}$ & 4.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-6}$ & 8.8$\times10^{37}$ & 1.2$\times10^{-2}$\\
0.20 & M & -0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.7$\times10^{-8}$ & 5.4$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.0$\times10^{-8}$ & 8.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.5$\times10^{-8}$ & 5.2$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.7$\times10^{-8}$ & 8.2$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 1.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.1$\times10^{-8}$ & 4.9$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.0$\times10^{-8}$ & 7.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-8}$ & 4.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-8}$ & 7.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-8}$ & 4.3$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 6.9$\times10^{37}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
0.20 & M & -0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 9.2$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 3.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-7}$ & 5.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-7}$ & 9.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.8$\times10^{-8}$ & 9.0$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 3.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-7}$ & 4.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-7}$ & 8.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.6$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-7}$ & 4.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 8.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 8.1$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 4.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 7.9$\times10^{36}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 4.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & -0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 7.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
0.20 & M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.4$\times10^{-8}$ & 5.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.3$\times10^{-7}$ & 8.9$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.2$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.1$\times10^{-8}$ & 5.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 1.5$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.7$\times10^{-8}$ & 4.8$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.3$\times10^{-8}$ & 4.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.0$\times10^{-8}$ & 4.2$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.0 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &1.9$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
0.20 & M & 0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.0$\times10^{-8}$ & 3.3$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 10.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-7}$ & 2.7$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-7}$ & 8.5$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.2$\times10^{-7}$ & 2.6$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.7$\times10^{-8}$ & 3.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &9.6$\times10^{-8}$ & 7.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.6$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.9$\times10^{-7}$ & 2.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.4$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.6$\times10^{-8}$ & 7.0$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-7}$ & 2.2$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.1$\times10^{-8}$ & 6.7$\times10^{37}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
0.20 & M & 0.94 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.6$\times10^{-9}$ & 4.1$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.4$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &4.0$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 10.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.8$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.5$\times10^{-9}$ & 4.1$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.9$\times10^{-8}$ & 1.9$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 30.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.8$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.3$\times10^{-9}$ & 4.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &3.8$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.7$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &8.1$\times10^{-9}$ & 3.9$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.1$\times10^{-8}$ & 10.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.7$\times10^{-8}$ & 3.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.7$\times10^{-9}$ & 3.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.1$\times10^{-8}$ & 9.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
0.20 & M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &6.9$\times10^{-8}$ & 3.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Frankfurt_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|cccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Frankfurt Thermal Models}
\label{tab:frankfurtPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{$L_X$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.0$\times10^{-8}$ & 1.5$\times10^{36}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 10.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 2.2$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-6}$ & 4.2$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.0$\times10^{-6}$ & 6.4$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.7$\times10^{-8}$ & 1.5$\times10^{36}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 30.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 2.1$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.7$\times10^{-6}$ & 4.3$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.3$\times10^{-6}$ & 6.8$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.4$\times10^{-8}$ & 1.4$\times10^{36}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 2.0$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-6}$ & 4.0$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.1$\times10^{-6}$ & 6.4$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.4$\times10^{-8}$ & 1.4$\times10^{36}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 1.9$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.4$\times10^{-6}$ & 3.9$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.1$\times10^{-6}$ & 6.5$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.2$\times10^{-8}$ & 1.4$\times10^{36}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 1.9$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-6}$ & 4.0$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.3$\times10^{-6}$ & 6.8$\times10^{37}$ & 3.3$\times10^{-3}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.9$\times10^{-8}$ & 2.8$\times10^{35}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 10.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 8.9$\times10^{36}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &$0.0$ & $0.0$ & $0.0$\\
S & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.1$\times10^{-6}$ & 2.8$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.8$\times10^{-8}$ & 2.7$\times10^{35}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 30.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-6}$ & 8.9$\times10^{36}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &4.3$\times10^{-6}$ & 2.0$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-6}$ & 3.0$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-8}$ & 2.7$\times10^{35}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 50.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-6}$ & 8.7$\times10^{36}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 50.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &4.2$\times10^{-6}$ & 1.9$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.5$\times10^{-6}$ & 2.9$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &5.8$\times10^{-8}$ & 2.7$\times10^{35}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 70.0 & 10.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 8.9$\times10^{36}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 70.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.3$\times10^{-6}$ & 1.9$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.8$\times10^{-6}$ & 3.0$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.7$\times10^{-8}$ & 2.6$\times10^{35}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 90.0 & 10.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 9.0$\times10^{36}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 90.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.4$\times10^{-6}$ & 2.0$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & -0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.2$\times10^{-6}$ & 3.2$\times10^{37}$ & 9.2$\times10^{-4}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 5.0$\times10^{34}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 10.0 & 10.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 1.5$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-6}$ & 4.8$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.0$\times10^{-6}$ & 7.9$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 4.9$\times10^{34}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 30.0 & 10.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 1.5$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-6}$ & 4.6$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 30.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-6}$ & 7.4$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 4.8$\times10^{34}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 50.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.1$\times10^{-6}$ & 1.5$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 50.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-6}$ & 4.7$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-6}$ & 7.5$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 70.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.5$\times10^{-8}$ & 4.8$\times10^{34}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 70.0 & 10.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-6}$ & 1.6$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 70.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 4.9$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 70.0 & 160.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.2$\times10^{-6}$ & 8.2$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.5$\times10^{-8}$ & 4.7$\times10^{34}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 90.0 & 10.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-6}$ & 1.7$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 90.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-6}$ & 5.1$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.0 & 90.0 & 160.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-6}$ & 8.6$\times10^{36}$ & 2.7$\times10^{-4}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-8}$ & 3.0$\times10^{35}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.3$\times10^{-7}$ & 4.5$\times10^{36}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.3$\times10^{-6}$ & 1.5$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &2.5$\times10^{-6}$ & 3.0$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 2.9$\times10^{35}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 30.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-7}$ & 4.4$\times10^{36}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.2$\times10^{-6}$ & 1.5$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &2.4$\times10^{-6}$ & 2.9$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 2.9$\times10^{35}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 50.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 4.2$\times10^{36}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 1.5$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-6}$ & 3.0$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.9$\times10^{-8}$ & 2.8$\times10^{35}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 70.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 4.2$\times10^{36}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 70.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 1.5$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-6}$ & 3.2$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.9$\times10^{-8}$ & 2.8$\times10^{35}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 90.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-7}$ & 4.3$\times10^{36}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 1.5$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-6}$ & 3.2$\times10^{37}$ & 2.8$\times10^{-3}$\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.4$\times10^{-9}$ & 2.9$\times10^{35}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 10.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 4.2$\times10^{36}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.2$\times10^{-7}$ & 2.3$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-6}$ & 4.1$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.2$\times10^{-9}$ & 2.8$\times10^{35}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 30.0 & 10.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-7}$ & 4.1$\times10^{36}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 30.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-7}$ & 2.6$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 30.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-6}$ & 4.6$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.9$\times10^{-9}$ & 2.7$\times10^{35}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass &1.0$\times10^{-7}$ & 4.1$\times10^{36}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.8$\times10^{-7}$ & 2.9$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 50.0 & 160.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-6}$ & 5.5$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.8$\times10^{-9}$ & 2.6$\times10^{35}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 4.3$\times10^{36}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.8$\times10^{-7}$ & 2.9$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 6.0$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.7$\times10^{-9}$ & 2.6$\times10^{35}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-7}$ & 4.5$\times10^{36}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-7}$ & 2.9$\times10^{37}$ & 7.6$\times10^{-3}$\\
S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 6.1$\times10^{37}$ & 7.6$\times10^{-3}$\\
M & -0.94 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.5$\times10^{-8}$ & 8.5$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.2$\times10^{-8}$ & 2.2$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.7$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.9$\times10^{-7}$ & 7.0$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.4$\times10^{-8}$ & 8.2$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.9$\times10^{-8}$ & 2.1$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.5$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 6.7$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.2$\times10^{-8}$ & 7.8$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.2$\times10^{-8}$ & 1.9$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 3.2$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-7}$ & 6.1$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.0$\times10^{-8}$ & 7.3$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.3$\times10^{-8}$ & 1.7$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.9$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 5.5$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.8$\times10^{-8}$ & 6.9$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.9$\times10^{-8}$ & 1.6$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.7$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 5.3$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-8}$ & 1.4$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.5$\times10^{-8}$ & 4.1$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 10.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 6.6$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.0$\times10^{-8}$ & 1.4$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.2$\times10^{-8}$ & 4.0$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 6.4$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-8}$ & 1.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &8.5$\times10^{-8}$ & 3.7$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 5.9$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.7$\times10^{-8}$ & 1.2$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.7$\times10^{-8}$ & 3.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 5.4$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 9.7$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-8}$ & 1.2$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.5$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 5.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 9.7$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.7$\times10^{-8}$ & 4.8$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-8}$ & 1.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.5$\times10^{-8}$ & 4.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 7.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.1$\times10^{-8}$ & 4.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.5$\times10^{-8}$ & 6.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.1$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.7$\times10^{-8}$ & 4.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.9$\times10^{-8}$ & 6.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.0$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-8}$ & 1.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-8}$ & 3.9$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &8.7$\times10^{-8}$ & 6.2$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.0$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.9$\times10^{-8}$ & 9.1$\times10^{36}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.3$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &8.9$\times10^{-8}$ & 4.5$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 7.7$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.9$\times10^{-8}$ & 8.9$\times10^{36}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.1$\times10^{-8}$ & 2.5$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &8.6$\times10^{-8}$ & 4.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.5$\times10^{-7}$ & 7.5$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.8$\times10^{-8}$ & 8.7$\times10^{36}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.9$\times10^{-8}$ & 2.4$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &8.2$\times10^{-8}$ & 4.1$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.4$\times10^{-7}$ & 7.2$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.8$\times10^{-8}$ & 8.4$\times10^{36}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &4.6$\times10^{-8}$ & 2.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &7.9$\times10^{-8}$ & 3.9$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 7.0$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 7.8$\times10^{36}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &4.4$\times10^{-8}$ & 2.2$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-8}$ & 3.9$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 7.0$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & 0.94 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.0$\times10^{-9}$ & 2.4$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.1$\times10^{-8}$ & 6.4$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.6$\times10^{-8}$ & 1.1$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &6.2$\times10^{-8}$ & 1.9$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.9$\times10^{-9}$ & 2.4$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.1$\times10^{-8}$ & 6.3$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.6$\times10^{-8}$ & 1.1$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &6.2$\times10^{-8}$ & 1.8$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.8$\times10^{-9}$ & 2.3$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &2.0$\times10^{-8}$ & 6.0$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &3.5$\times10^{-8}$ & 1.0$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.2$\times10^{-8}$ & 1.8$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.5$\times10^{-9}$ & 2.2$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.9$\times10^{-8}$ & 5.7$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &3.4$\times10^{-8}$ & 1.0$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.3$\times10^{-8}$ & 1.9$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.2$\times10^{-9}$ & 2.2$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.9$\times10^{-8}$ & 5.7$\times10^{37}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.5$\times10^{-8}$ & 1.0$\times10^{38}$ & 5.6$\times10^{-1}$\\
M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.5$\times10^{-8}$ & 1.9$\times10^{38}$ & 5.6$\times10^{-1}$\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Frankfurt_k5_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|ccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Frankfurt $\kappa$ 5 Models}
\label{tab:frankfurtk5PF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.9$\times10^{-9}$ & 1.9$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.3$\times10^{-8}$ & 2.0$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.1$\times10^{-7}$ & 9.0$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-6}$ & 2.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.6$\times10^{-9}$ & 1.9$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.9$\times10^{-8}$ & 1.9$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-7}$ & 8.3$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 2.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.4$\times10^{-9}$ & 1.8$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.4$\times10^{-8}$ & 1.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 7.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.2$\times10^{-9}$ & 1.8$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.0$\times10^{-8}$ & 1.7$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-7}$ & 6.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 70.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.0$\times10^{-9}$ & 1.7$\times10^{35}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-8}$ & 1.7$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.0$\times10^{-7}$ & 6.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & -0.94 & 90.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-6}$ & 2.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.5$\times10^{-8}$ & 2.8$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.2$\times10^{-7}$ & 3.2$\times10^{36}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.2$\times10^{-6}$ & 1.4$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.1$\times10^{-6}$ & 3.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.4$\times10^{-8}$ & 2.7$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 10.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.0$\times10^{-7}$ & 3.1$\times10^{36}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.1$\times10^{-6}$ & 1.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &5.3$\times10^{-6}$ & 3.3$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.2$\times10^{-8}$ & 2.6$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.7$\times10^{-7}$ & 2.9$\times10^{36}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 1.2$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.0$\times10^{-6}$ & 3.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.1$\times10^{-8}$ & 2.6$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-7}$ & 2.8$\times10^{36}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 70.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-6}$ & 2.9$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.0$\times10^{-8}$ & 2.5$\times10^{35}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.4$\times10^{-7}$ & 2.7$\times10^{36}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & -0.5 & 90.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-6}$ & 3.0$\times10^{37}$ & 1.2$\times10^{-3}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.7$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 10.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-7}$ & 6.8$\times10^{35}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.4$\times10^{-7}$ & 2.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-6}$ & 5.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.6$\times10^{-8}$ & 8.4$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.7$\times10^{-7}$ & 6.3$\times10^{35}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.5$\times10^{-7}$ & 2.0$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 4.6$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.2$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.5$\times10^{-7}$ & 5.8$\times10^{35}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &7.4$\times10^{-7}$ & 1.7$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-6}$ & 3.9$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-8}$ & 7.9$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 5.3$\times10^{35}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &6.3$\times10^{-7}$ & 1.5$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 70.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-8}$ & 7.7$\times10^{34}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 4.9$\times10^{35}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.7$\times10^{-7}$ & 1.3$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.0 & 90.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-6}$ & 3.2$\times10^{36}$ & 4.5$\times10^{-4}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.3$\times10^{-7}$ & 2.8$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-6}$ & 2.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.2$\times10^{-6}$ & 6.9$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.6$\times10^{-6}$ & 1.2$\times10^{38}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.3$\times10^{-7}$ & 2.7$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.5$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.2$\times10^{-6}$ & 6.8$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.8$\times10^{-6}$ & 1.2$\times10^{38}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 2.6$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-6}$ & 2.3$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.9$\times10^{-6}$ & 6.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.2$\times10^{-6}$ & 1.1$\times10^{38}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 2.5$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &9.9$\times10^{-7}$ & 2.1$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.6$\times10^{-6}$ & 5.6$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail & Fail & Fail &4.8$\times10^{-6}$ & 1.0$\times10^{38}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 2.4$\times10^{36}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &9.2$\times10^{-7}$ & 2.0$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail & Fail & Fail &2.4$\times10^{-6}$ & 5.2$\times10^{37}$ & 4.2$\times10^{-3}$\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-6}$ & 1.0$\times10^{38}$ & 4.2$\times10^{-3}$\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &7.3$\times10^{-9}$ & 4.4$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 10.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.5$\times10^{-8}$ & 3.3$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.2$\times10^{-7}$ & 1.3$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.3$\times10^{-7}$ & 4.4$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.1$\times10^{-9}$ & 4.3$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.1$\times10^{-8}$ & 3.0$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.0$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 30.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &6.7$\times10^{-7}$ & 4.1$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &6.9$\times10^{-9}$ & 4.1$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &4.5$\times10^{-8}$ & 2.7$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 9.8$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.3$\times10^{-7}$ & 3.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &4.0$\times10^{-8}$ & 2.4$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 7.6$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 2.1$\times10^{37}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-9}$ & 4.0$\times10^{35}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &3.9$\times10^{-8}$ & 2.3$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 7.5$\times10^{36}$ & 1.2$\times10^{-2}$\\
S & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.7$\times10^{-7}$ & 2.2$\times10^{37}$ & 1.2$\times10^{-2}$\\
M & -0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.4$\times10^{-8}$ & 5.2$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.9$\times10^{-8}$ & 8.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-8}$ & 1.7$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.2$\times10^{-8}$ & 4.9$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.5$\times10^{-8}$ & 8.1$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-8}$ & 1.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-8}$ & 4.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-8}$ & 7.4$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.4$\times10^{-8}$ & 4.2$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.0$\times10^{-8}$ & 6.6$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-7}$ & 1.1$\times10^{38}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-8}$ & 1.5$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.0$\times10^{-8}$ & 3.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.3$\times10^{-8}$ & 6.0$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 9.8$\times10^{37}$ & 1.8$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &3.8$\times10^{-8}$ & 9.0$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 2.9$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.1$\times10^{-7}$ & 5.0$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.7$\times10^{-7}$ & 8.8$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 8.7$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.8$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-7}$ & 4.7$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 8.4$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 8.2$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 2.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.8$\times10^{-7}$ & 4.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-7}$ & 7.6$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.3$\times10^{-8}$ & 7.7$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail &9.3$\times10^{-8}$ & 2.2$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.6$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-7}$ & 6.3$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-8}$ & 7.5$\times10^{36}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail &9.0$\times10^{-8}$ & 2.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.5$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & -0.5 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 6.1$\times10^{37}$ & 4.6$\times10^{-2}$\\
M & 0.0 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.0$\times10^{-8}$ & 5.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 8.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass &2.0$\times10^{-7}$ & 1.4$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.4$\times10^{-8}$ & 1.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.6$\times10^{-8}$ & 4.7$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 8.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 1.3$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.3$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.2$\times10^{-8}$ & 4.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 7.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.2$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.2$\times10^{-8}$ & 1.6$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail &5.6$\times10^{-8}$ & 4.0$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &9.1$\times10^{-8}$ & 6.5$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.1$\times10^{37}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.0$\times10^{-8}$ & 1.4$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &4.6$\times10^{-8}$ & 3.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 5.1$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.3$\times10^{36}$ & 1.4$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 8.4$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.0$\times10^{-7}$ & 2.5$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 3.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.8$\times10^{-8}$ & 8.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.3$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-7}$ & 2.4$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 2.9$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &9.0$\times10^{-8}$ & 7.4$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.2$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 2.1$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &8.0$\times10^{-8}$ & 6.6$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.0$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 1.8$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.0$\times10^{-8}$ & 2.5$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &7.4$\times10^{-8}$ & 6.1$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 9.7$\times10^{37}$ & 1.6$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 1.7$\times10^{38}$ & 1.6$\times10^{-1}$\\
M & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &9.1$\times10^{-9}$ & 4.4$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 1.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.8$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.5$\times10^{-8}$ & 3.1$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &9.0$\times10^{-9}$ & 4.3$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail &3.7$\times10^{-8}$ & 1.8$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail &6.2$\times10^{-8}$ & 3.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.7$\times10^{-9}$ & 4.2$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail &2.0$\times10^{-8}$ & 9.7$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.3$\times10^{-8}$ & 1.6$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 2.7$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &8.3$\times10^{-9}$ & 4.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.8$\times10^{-8}$ & 8.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.9$\times10^{-8}$ & 1.4$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &4.9$\times10^{-8}$ & 2.3$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &7.9$\times10^{-9}$ & 3.8$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.7$\times10^{-8}$ & 8.0$\times10^{37}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.6$\times10^{-8}$ & 1.2$\times10^{38}$ & 9.3$\times10^{-1}$\\
M & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &4.2$\times10^{-8}$ & 2.0$\times10^{38}$ & 9.3$\times10^{-1}$\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Hamr_All_Tilts.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|cccc|c|cccccc|c|c|c}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, \hamr Tilted Models}
\label{tab:TiltedhamrPF}
\tablehead{ \colhead{Tilt}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
}
\startdata
0 & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
0 & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
0 & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
0 & 0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
0 & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
0 & 0.94 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
0 & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
0 & 0.94 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
0 & 0.94 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
30 & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass\\
30 & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
30 & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
30 & 0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
30 & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
30 & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass\\
30 & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
30 & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
30 & 0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
60 & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
60 & 0.94 & 10.0 & 40.0 & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
60 & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
60 & 0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass\\
60 & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass\\
60 & 0.94 & 50.0 & 160.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
60 & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass\\
60 & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
60 & 0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Hamr_Nonthermal_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|ccc|c|cccccc|c|c|c}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, \hamr Nonthermal Powerlaw Models}
\label{tab:hamr_nth}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.94 & 10.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.94 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass\\
S & -0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.94 & 50.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.94 & 50.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.94 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.94 & 90.0 & 40.0 & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.94 & 90.0 & 160.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
S & -0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.5 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & -0.5 & 90.0 & 1.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.5 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass\\
S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & 0.0 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 90.0 & 1.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 90.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.0 & 90.0 & 160.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.5 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
S & 0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
S & 0.94 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass\\
S & 0.94 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.94 & 90.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
S & 0.94 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
S & 0.94 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
M & -0.94 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.94 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.94 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 50.0 & 1.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & -0.5 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 90.0 & 1.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
M & 0.0 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 90.0 & 1.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail\\
M & 0.0 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.0 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 10.0 & 1.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass\\
M & 0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 50.0 & 1.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass\\
M & 0.5 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 90.0 & 1.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail\\
M & 0.5 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
M & 0.94 & 50.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail\\
M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail\\
M & 0.94 & 90.0 & 40.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
M & 0.94 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Hamr_Thermal_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|cccc|c|ccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, \hamr Thermal Models}
\label{tab:ThamrPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{$L_X$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$L_{bol}/(\dot{M} c^{2})$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.1$\times10^{-7}$ & 6.3$\times10^{-5}$ & 1.9$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 10.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &2.8$\times10^{-5}$ & 2.2$\times10^{-5}$ & 1.2$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-4}$ & 2.5 & 6.4$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.6$\times10^{-7}$ & 5.7$\times10^{-5}$ & 1.6$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 50.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-5}$ & 2.5$\times10^{-5}$ & 1.5$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 50.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-4}$ & 9.4$\times10^{-2}$ & 9.6$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 90.0 & 1.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-7}$ & 6.3$\times10^{-5}$ & 1.8$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 90.0 & 40.0 & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &4.0$\times10^{-5}$ & 3.1$\times10^{-5}$ & 1.8$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-4}$ & 9.4$\times10^{-4}$ & 1.4$\times10^{39}$ & 8.7$\times10^{-4}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-7}$ & 2.1$\times10^{-4}$ & 2.8$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 10.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.5$\times10^{-6}$ & 4.7$\times10^{-5}$ & 3.9$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-6}$ & 2.1$\times10^{-5}$ & 7.4$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.6$\times10^{-7}$ & 1.8$\times10^{-4}$ & 2.4$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.2$\times10^{-6}$ & 4.1$\times10^{-5}$ & 3.3$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 160.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.5$\times10^{-6}$ & 1.8$\times10^{-5}$ & 6.9$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 1.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.7$\times10^{-4}$ & 2.3$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &2.0$\times10^{-6}$ & 3.8$\times10^{-5}$ & 3.1$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.4$\times10^{-6}$ & 1.7$\times10^{-5}$ & 6.8$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 3.3$\times10^{-4}$ & 1.2$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-6}$ & 3.8$\times10^{-5}$ & 1.6$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.5$\times10^{-6}$ & 1.6$\times10^{-5}$ & 2.6$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.1$\times10^{-7}$ & 2.9$\times10^{-4}$ & 1.1$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-6}$ & 3.8$\times10^{-5}$ & 1.6$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 160.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.6$\times10^{-6}$ & 1.7$\times10^{-5}$ & 2.7$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 1.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &10.0$\times10^{-8}$ & 2.7$\times10^{-4}$ & 1.0$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass &1.7$\times10^{-6}$ & 4.1$\times10^{-5}$ & 1.8$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.1$\times10^{-6}$ & 2.0$\times10^{-5}$ & 3.3$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &7.0$\times10^{-8}$ & 7.4$\times10^{-4}$ & 1.3$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 10.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.7$\times10^{-6}$ & 1.1$\times10^{-4}$ & 3.2$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.4$\times10^{-6}$ & 3.2$\times10^{-5}$ & 6.6$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.2$\times10^{-8}$ & 9.2$\times10^{-4}$ & 1.2$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.8$\times10^{-6}$ & 1.1$\times10^{-4}$ & 3.4$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 160.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &4.0$\times10^{-6}$ & 3.7$\times10^{-5}$ & 7.7$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.8$\times10^{-8}$ & 6.2$\times10^{-4}$ & 1.1$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-6}$ & 1.1$\times10^{-4}$ & 3.4$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 160.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-6}$ & 3.6$\times10^{-5}$ & 7.5$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.8$\times10^{-8}$ & 4.3$\times10^{-3}$ & 2.9$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 10.0 & 40.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &7.5$\times10^{-7}$ & 6.4$\times10^{-4}$ & 7.8$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.6$\times10^{-6}$ & 1.6$\times10^{-4}$ & 1.7$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 50.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.5$\times10^{-8}$ & 3.7$\times10^{-3}$ & 2.6$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 50.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.4$\times10^{-7}$ & 7.2$\times10^{-4}$ & 8.7$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 50.0 & 160.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.9$\times10^{-6}$ & 1.9$\times10^{-4}$ & 2.0$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 3.4$\times10^{-3}$ & 2.4$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.2$\times10^{-7}$ & 7.0$\times10^{-4}$ & 8.5$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.94 & 90.0 & 160.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass &2.0$\times10^{-6}$ & 2.0$\times10^{-4}$ & 2.1$\times10^{38}$ & 2.0$\times10^{-2}$\\
M & -0.94 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.8$\times10^{-8}$ & 1.0$\times10^{-2}$ & 4.8$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.9$\times10^{-8}$ & 1.7$\times10^{-3}$ & 10.0$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 6.6$\times10^{-4}$ & 1.7$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.2$\times10^{-8}$ & 8.8$\times10^{-3}$ & 4.2$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.7$\times10^{-8}$ & 1.5$\times10^{-3}$ & 8.8$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 5.9$\times10^{-4}$ & 1.5$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.9$\times10^{-8}$ & 8.2$\times10^{-3}$ & 3.9$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.3$\times10^{-8}$ & 1.4$\times10^{-3}$ & 8.3$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.94 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 5.7$\times10^{-4}$ & 1.4$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-8}$ & 6.4$\times10^{-3}$ & 3.8$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 1.5$\times10^{-3}$ & 8.7$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-7}$ & 7.0$\times10^{-4}$ & 1.6$\times10^{38}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 5.6$\times10^{-3}$ & 3.4$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.3$\times10^{-3}$ & 7.8$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 6.2$\times10^{-4}$ & 1.4$\times10^{38}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.1$\times10^{-8}$ & 5.0$\times10^{-3}$ & 3.0$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.2$\times10^{-3}$ & 7.2$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 6.0$\times10^{-4}$ & 1.3$\times10^{38}$ & 1.2$\times10^{-1}$\\
M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 4.8$\times10^{-3}$ & 1.4$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 1.2$\times10^{-3}$ & 3.8$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 5.5$\times10^{-4}$ & 6.5$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &3.4$\times10^{-8}$ & 4.3$\times10^{-3}$ & 1.3$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &8.5$\times10^{-8}$ & 1.0$\times10^{-3}$ & 3.2$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 4.7$\times10^{-4}$ & 5.5$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.0$\times10^{-8}$ & 3.8$\times10^{-3}$ & 1.1$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.4$\times10^{-8}$ & 8.8$\times10^{-4}$ & 2.8$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 4.1$\times10^{-4}$ & 4.8$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.8$\times10^{-8}$ & 1.2$\times10^{-2}$ & 5.9$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.2$\times10^{-7}$ & 2.7$\times10^{-3}$ & 1.9$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-7}$ & 1.2$\times10^{-3}$ & 3.6$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &3.5$\times10^{-8}$ & 1.1$\times10^{-2}$ & 5.4$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 2.6$\times10^{-3}$ & 1.8$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 1.1$\times10^{-3}$ & 3.4$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.1$\times10^{-8}$ & 9.2$\times10^{-3}$ & 4.8$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-7}$ & 2.4$\times10^{-3}$ & 1.7$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 1.1$\times10^{-3}$ & 3.3$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.94 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.8$\times10^{-8}$ & 2.7$\times10^{-2}$ & 1.1$\times10^{38}$ & 1.2\\
M & 0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.3$\times10^{-8}$ & 4.8$\times10^{-3}$ & 2.7$\times10^{38}$ & 1.2\\
M & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.6$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.7$\times10^{38}$ & 1.2\\
M & 0.94 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-8}$ & 2.7$\times10^{-2}$ & 1.1$\times10^{38}$ & 1.2\\
M & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &4.0$\times10^{-8}$ & 4.7$\times10^{-3}$ & 2.5$\times10^{38}$ & 1.2\\
M & 0.94 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.4$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.6$\times10^{38}$ & 1.2\\
M & 0.94 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-8}$ & 2.6$\times10^{-2}$ & 9.6$\times10^{37}$ & 1.2\\
M & 0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 4.5$\times10^{-3}$ & 2.3$\times10^{38}$ & 1.2\\
M & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.5$\times10^{38}$ & 1.2\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Hamr_varkappa_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|cccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, \hamr Variable $\kappa$ Models}
\label{tab:tab:vkhamrPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{$L_X$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$L_{bol}/(\dot{M} c^{2})$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.93 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.0$\times10^{-7}$ & 2.6$\times10^{-3}$ & 1.8$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 10.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-6}$ & 9.0$\times10^{-5}$ & 2.2$\times10^{37}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 10.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-5}$ & 7.9$\times10^{-5}$ & 1.8$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 10.0 & 160.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.4$\times10^{-3}$ & 3.5$\times10^{-2}$ & 2.4$\times10^{40}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-7}$ & 2.5$\times10^{-3}$ & 1.7$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 30.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-6}$ & 8.9$\times10^{-5}$ & 2.2$\times10^{37}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 30.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.2$\times10^{-5}$ & 8.4$\times10^{-5}$ & 1.9$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-3}$ & 6.7$\times10^{-1}$ & 6.9$\times10^{39}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 50.0 & 1.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.6$\times10^{-7}$ & 2.4$\times10^{-3}$ & 1.6$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 50.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-6}$ & 9.0$\times10^{-5}$ & 2.2$\times10^{37}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 50.0 & 40.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &4.3$\times10^{-5}$ & 8.2$\times10^{-5}$ & 1.9$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.8$\times10^{-4}$ & 3.8$\times10^{-2}$ & 2.6$\times10^{39}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 70.0 & 1.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-7}$ & 2.4$\times10^{-3}$ & 1.7$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-6}$ & 9.5$\times10^{-5}$ & 2.4$\times10^{37}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.5$\times10^{-5}$ & 9.2$\times10^{-5}$ & 2.0$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.1$\times10^{-4}$ & 2.7$\times10^{-2}$ & 1.8$\times10^{39}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-7}$ & 2.5$\times10^{-3}$ & 1.7$\times10^{36}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 90.0 & 10.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-6}$ & 1.0$\times10^{-4}$ & 2.5$\times10^{37}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-5}$ & 9.5$\times10^{-5}$ & 2.1$\times10^{38}$ & 8.7$\times10^{-4}$\\
S & -0.93 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-4}$ & 6.8$\times10^{-3}$ & 1.6$\times10^{39}$ & 8.7$\times10^{-4}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-7}$ & 4.1$\times10^{-3}$ & 2.8$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.5$\times10^{-7}$ & 4.1$\times10^{-4}$ & 1.5$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 10.0 & 40.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.4$\times10^{-6}$ & 1.9$\times10^{-4}$ & 3.7$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-6}$ & 5.5$\times10^{-5}$ & 7.3$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-7}$ & 3.8$\times10^{-3}$ & 2.6$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.8$\times10^{-7}$ & 3.8$\times10^{-4}$ & 1.4$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 30.0 & 40.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-6}$ & 1.8$\times10^{-4}$ & 3.5$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 30.0 & 160.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &4.4$\times10^{-6}$ & 5.5$\times10^{-5}$ & 6.9$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.6$\times10^{-7}$ & 3.6$\times10^{-3}$ & 2.4$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.0$\times10^{-7}$ & 3.4$\times10^{-4}$ & 1.2$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.0$\times10^{-6}$ & 1.5$\times10^{-4}$ & 3.2$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.2$\times10^{-6}$ & 4.5$\times10^{-5}$ & 6.4$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.3$\times10^{-3}$ & 2.3$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-7}$ & 3.2$\times10^{-4}$ & 1.2$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.0$\times10^{-6}$ & 1.6$\times10^{-4}$ & 3.1$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &4.3$\times10^{-6}$ & 4.6$\times10^{-5}$ & 6.5$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-7}$ & 3.3$\times10^{-3}$ & 2.2$\times10^{36}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.4$\times10^{-7}$ & 3.2$\times10^{-4}$ & 1.1$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.9$\times10^{-6}$ & 1.5$\times10^{-4}$ & 3.0$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & -0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &4.2$\times10^{-6}$ & 4.5$\times10^{-5}$ & 6.4$\times10^{37}$ & 3.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-7}$ & 7.8$\times10^{-3}$ & 1.5$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &7.6$\times10^{-7}$ & 4.3$\times10^{-4}$ & 7.9$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 40.0 & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-6}$ & 2.0$\times10^{-4}$ & 1.7$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.7$\times10^{-6}$ & 3.3$\times10^{14}$ & 2.8$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.4$\times10^{-7}$ & 7.4$\times10^{-3}$ & 1.4$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 30.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &6.9$\times10^{-7}$ & 3.9$\times10^{-4}$ & 7.3$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.5$\times10^{-6}$ & 1.8$\times10^{-4}$ & 1.6$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 30.0 & 160.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.5$\times10^{-6}$ & 4.3$\times10^{6}$ & 2.6$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 6.8$\times10^{-3}$ & 1.3$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-7}$ & 3.7$\times10^{-4}$ & 7.0$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.7$\times10^{-6}$ & 2.0$\times10^{-4}$ & 1.7$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.8$\times10^{-6}$ & 1.7$\times10^{9}$ & 2.9$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 6.4$\times10^{-3}$ & 1.3$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 70.0 & 10.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &6.6$\times10^{-7}$ & 3.9$\times10^{-4}$ & 6.9$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 70.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.8$\times10^{-6}$ & 2.1$\times10^{-4}$ & 1.8$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.2$\times10^{-6}$ & 2.0$\times10^{8}$ & 3.4$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 6.2$\times10^{-3}$ & 1.2$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 10.0 & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.6$\times10^{-7}$ & 3.8$\times10^{-4}$ & 6.9$\times10^{36}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.8$\times10^{-6}$ & 2.1$\times10^{-4}$ & 1.9$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.0 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.4$\times10^{-6}$ & 9.4$\times10^{7}$ & 3.5$\times10^{37}$ & 2.0$\times10^{-3}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.8$\times10^{-8}$ & 1.2$\times10^{-2}$ & 1.3$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.8$\times10^{-7}$ & 7.7$\times10^{-4}$ & 7.2$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 10.0 & 40.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.7$\times10^{-6}$ & 4.3$\times10^{-4}$ & 3.2$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-6}$ & 9.2$\times10^{-5}$ & 6.7$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.3$\times10^{-8}$ & 1.1$\times10^{-2}$ & 1.2$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 30.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-7}$ & 7.2$\times10^{-4}$ & 6.7$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-6}$ & 4.2$\times10^{-4}$ & 3.1$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 30.0 & 160.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-6}$ & 9.2$\times10^{-5}$ & 6.7$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.0$\times10^{-8}$ & 1.1$\times10^{-2}$ & 1.2$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 10.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &3.3$\times10^{-7}$ & 6.7$\times10^{-4}$ & 6.3$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.7$\times10^{-6}$ & 4.3$\times10^{-4}$ & 3.2$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 9.9$\times10^{-5}$ & 7.2$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.7$\times10^{-8}$ & 10.0$\times10^{-3}$ & 1.1$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-7}$ & 6.7$\times10^{-4}$ & 6.2$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.6$\times10^{-6}$ & 4.2$\times10^{-4}$ & 3.1$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.7$\times10^{-6}$ & 1.2$\times10^{-4}$ & 7.1$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.6$\times10^{-8}$ & 9.8$\times10^{-3}$ & 1.1$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.3$\times10^{-7}$ & 6.7$\times10^{-4}$ & 6.3$\times10^{36}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &1.6$\times10^{-6}$ & 4.1$\times10^{-4}$ & 3.0$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-6}$ & 1.2$\times10^{-4}$ & 7.0$\times10^{37}$ & 3.7$\times10^{-3}$\\
S & 0.93 & 10.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.8$\times10^{-8}$ & 7.2$\times10^{-2}$ & 2.9$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-7}$ & 3.4$\times10^{-3}$ & 1.5$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 10.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &7.5$\times10^{-7}$ & 1.6$\times10^{-3}$ & 7.8$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 10.0 & 160.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.6$\times10^{-6}$ & 3.5$\times10^{-4}$ & 1.6$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 30.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.7$\times10^{-8}$ & 6.8$\times10^{-2}$ & 2.8$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 30.0 & 10.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 3.1$\times10^{-3}$ & 1.4$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 30.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &7.4$\times10^{-7}$ & 1.6$\times10^{-3}$ & 7.7$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 30.0 & 160.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.6$\times10^{-6}$ & 3.5$\times10^{-4}$ & 1.6$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 6.0$\times10^{-2}$ & 2.5$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 50.0 & 10.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Pass &1.2$\times10^{-7}$ & 2.8$\times10^{-3}$ & 1.2$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 50.0 & 40.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &7.8$\times10^{-7}$ & 1.7$\times10^{-3}$ & 8.1$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 50.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &1.7$\times10^{-6}$ & 3.9$\times10^{-4}$ & 1.8$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 70.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 5.4$\times10^{-2}$ & 2.4$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 70.0 & 10.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 2.7$\times10^{-3}$ & 1.2$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 70.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.7$\times10^{-7}$ & 1.7$\times10^{-3}$ & 8.0$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 70.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-6}$ & 4.0$\times10^{-4}$ & 1.9$\times10^{38}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 5.5$\times10^{-2}$ & 2.4$\times10^{36}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 90.0 & 10.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 2.8$\times10^{-3}$ & 1.2$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 90.0 & 40.0 & Fail & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.6$\times10^{-7}$ & 1.7$\times10^{-3}$ & 7.9$\times10^{37}$ & 2.0$\times10^{-2}$\\
S & 0.93 & 90.0 & 160.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-6}$ & 4.0$\times10^{-4}$ & 1.9$\times10^{38}$ & 2.0$\times10^{-2}$\\
M & -0.93 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.7$\times10^{-8}$ & 6.7$\times10^{-2}$ & 4.7$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.7$\times10^{-8}$ & 8.8$\times10^{-3}$ & 6.7$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 10.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.7$\times10^{-8}$ & 2.6$\times10^{-3}$ & 9.8$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 7.4$\times10^{-4}$ & 1.7$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.3$\times10^{-8}$ & 5.1$\times10^{-2}$ & 4.4$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-8}$ & 8.4$\times10^{-3}$ & 6.3$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 30.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.1$\times10^{-8}$ & 2.4$\times10^{-3}$ & 9.1$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 6.9$\times10^{-4}$ & 1.6$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.1$\times10^{-8}$ & 4.9$\times10^{-2}$ & 4.1$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.9$\times10^{-8}$ & 7.9$\times10^{-3}$ & 5.9$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.6$\times10^{-8}$ & 2.3$\times10^{-3}$ & 8.6$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 6.4$\times10^{-4}$ & 1.5$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 70.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 5.4$\times10^{-2}$ & 3.9$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.5$\times10^{-8}$ & 7.7$\times10^{-3}$ & 5.5$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.1$\times10^{-8}$ & 2.1$\times10^{-3}$ & 8.1$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 6.0$\times10^{-4}$ & 1.4$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.8$\times10^{-8}$ & 4.5$\times10^{-2}$ & 3.8$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 6.3$\times10^{-3}$ & 5.4$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.0$\times10^{-8}$ & 2.1$\times10^{-3}$ & 8.0$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.93 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 6.1$\times10^{-4}$ & 1.4$\times10^{38}$ & 1.9$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.7$\times10^{-8}$ & 2.9$\times10^{-2}$ & 2.8$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-8}$ & 5.1$\times10^{-3}$ & 4.2$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 10.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-7}$ & 1.9$\times10^{-3}$ & 6.4$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-7}$ & 6.1$\times10^{-4}$ & 1.1$\times10^{38}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.5$\times10^{-8}$ & 3.2$\times10^{-2}$ & 2.7$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.8$\times10^{-8}$ & 4.6$\times10^{-3}$ & 4.0$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 1.8$\times10^{-3}$ & 6.1$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 5.8$\times10^{-4}$ & 1.0$\times10^{38}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.2$\times10^{-8}$ & 2.8$\times10^{-2}$ & 2.5$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-8}$ & 4.3$\times10^{-3}$ & 3.8$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.5$\times10^{-8}$ & 1.8$\times10^{-3}$ & 5.7$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 5.5$\times10^{-4}$ & 9.5$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 2.4$\times10^{-2}$ & 2.3$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.8$\times10^{-8}$ & 4.1$\times10^{-3}$ & 3.5$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.7$\times10^{-8}$ & 1.6$\times10^{-3}$ & 5.2$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 5.1$\times10^{-4}$ & 9.0$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-8}$ & 2.7$\times10^{-2}$ & 2.2$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.7$\times10^{-8}$ & 4.1$\times10^{-3}$ & 3.4$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.6$\times10^{-8}$ & 1.6$\times10^{-3}$ & 5.1$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 5.0$\times10^{-4}$ & 8.9$\times10^{37}$ & 1.2$\times10^{-1}$\\
M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &3.7$\times10^{-8}$ & 2.8$\times10^{-2}$ & 1.4$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.0$\times10^{-8}$ & 4.7$\times10^{-3}$ & 2.3$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.7$\times10^{-8}$ & 2.1$\times10^{-3}$ & 3.7$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 7.4$\times10^{-4}$ & 6.4$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &3.5$\times10^{-8}$ & 2.5$\times10^{-2}$ & 1.3$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.8$\times10^{-8}$ & 4.5$\times10^{-3}$ & 2.2$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &9.1$\times10^{-8}$ & 2.0$\times10^{-3}$ & 3.4$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 7.0$\times10^{-4}$ & 6.0$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &3.3$\times10^{-8}$ & 2.3$\times10^{-2}$ & 1.3$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-8}$ & 4.1$\times10^{-3}$ & 2.0$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.4$\times10^{-8}$ & 1.8$\times10^{-3}$ & 3.2$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 6.2$\times10^{-4}$ & 5.3$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &3.1$\times10^{-8}$ & 2.1$\times10^{-2}$ & 1.2$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.8$\times10^{-8}$ & 3.7$\times10^{-3}$ & 1.8$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.6$\times10^{-8}$ & 1.7$\times10^{-3}$ & 2.9$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 5.8$\times10^{-4}$ & 4.9$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-8}$ & 2.0$\times10^{-2}$ & 1.1$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-8}$ & 3.5$\times10^{-3}$ & 1.7$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 1.6$\times10^{-3}$ & 2.7$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-7}$ & 5.6$\times10^{-4}$ & 4.8$\times10^{37}$ & 7.3$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &2.9$\times10^{-8}$ & 5.5$\times10^{-2}$ & 4.5$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.9$\times10^{-8}$ & 8.2$\times10^{-3}$ & 7.7$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &8.5$\times10^{-8}$ & 3.1$\times10^{-3}$ & 1.3$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 9.4$\times10^{-4}$ & 2.4$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.8$\times10^{-8}$ & 5.4$\times10^{-2}$ & 4.4$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.8$\times10^{-8}$ & 9.1$\times10^{-3}$ & 7.5$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &8.3$\times10^{-8}$ & 3.0$\times10^{-3}$ & 1.3$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 9.1$\times10^{-4}$ & 2.3$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &2.7$\times10^{-8}$ & 5.1$\times10^{-2}$ & 4.3$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-8}$ & 7.9$\times10^{-3}$ & 7.1$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.8$\times10^{-8}$ & 2.9$\times10^{-3}$ & 1.2$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 8.8$\times10^{-4}$ & 2.2$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-8}$ & 4.7$\times10^{-2}$ & 4.0$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.3$\times10^{-8}$ & 7.7$\times10^{-3}$ & 6.8$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-8}$ & 2.7$\times10^{-3}$ & 1.2$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 8.5$\times10^{-4}$ & 2.2$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 9.5$\times10^{-2}$ & 3.8$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.1$\times10^{-8}$ & 7.8$\times10^{-3}$ & 6.3$\times10^{37}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 2.6$\times10^{-3}$ & 1.1$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 8.4$\times10^{-4}$ & 2.1$\times10^{38}$ & 3.0$\times10^{-1}$\\
M & 0.93 & 10.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.8$\times10^{-8}$ & 2.2$\times10^{-1}$ & 1.1$\times10^{38}$ & 1.2\\
M & 0.93 & 10.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.7$\times10^{-8}$ & 2.2$\times10^{-2}$ & 1.7$\times10^{38}$ & 1.2\\
M & 0.93 & 10.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.2$\times10^{-8}$ & 6.9$\times10^{-3}$ & 2.6$\times10^{38}$ & 1.2\\
M & 0.93 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.7$\times10^{38}$ & 1.2\\
M & 0.93 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.8$\times10^{-8}$ & 2.3$\times10^{-1}$ & 1.1$\times10^{38}$ & 1.2\\
M & 0.93 & 30.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.6$\times10^{-8}$ & 2.1$\times10^{-2}$ & 1.6$\times10^{38}$ & 1.2\\
M & 0.93 & 30.0 & 40.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.0$\times10^{-8}$ & 6.5$\times10^{-3}$ & 2.5$\times10^{38}$ & 1.2\\
M & 0.93 & 30.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.4$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.6$\times10^{38}$ & 1.2\\
M & 0.93 & 50.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-8}$ & 2.2$\times10^{-1}$ & 1.0$\times10^{38}$ & 1.2\\
M & 0.93 & 50.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &2.5$\times10^{-8}$ & 2.0$\times10^{-2}$ & 1.5$\times10^{38}$ & 1.2\\
M & 0.93 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 6.4$\times10^{-3}$ & 2.4$\times10^{38}$ & 1.2\\
M & 0.93 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 1.6$\times10^{-3}$ & 4.5$\times10^{38}$ & 1.2\\
M & 0.93 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-8}$ & 1.9$\times10^{-1}$ & 9.9$\times10^{37}$ & 1.2\\
M & 0.93 & 70.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.4$\times10^{-8}$ & 1.9$\times10^{-2}$ & 1.5$\times10^{38}$ & 1.2\\
M & 0.93 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 6.2$\times10^{-3}$ & 2.3$\times10^{38}$ & 1.2\\
M & 0.93 & 70.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-8}$ & 1.6$\times10^{-3}$ & 4.4$\times10^{38}$ & 1.2\\
M & 0.93 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-8}$ & 1.8$\times10^{-1}$ & 9.4$\times10^{37}$ & 1.2\\
M & 0.93 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.8$\times10^{-2}$ & 1.4$\times10^{38}$ & 1.2\\
M & 0.93 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.7$\times10^{-8}$ & 6.0$\times10^{-3}$ & 2.3$\times10^{38}$ & 1.2\\
M & 0.93 & 90.0 & 160.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 1.7$\times10^{-3}$ & 4.5$\times10^{38}$ & 1.2\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Illinois_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|cccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Illinois Thermal Models}
\label{tab:illinoisPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{$L_X$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$L_{bol}/(\dot{M} c^{2})$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
S & -0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.8$\times10^{-7}$ & 1.3$\times10^{-4}$ & 2.2$\times10^{36}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 10.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-6}$ & 3.3$\times10^{-5}$ & 2.7$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.8$\times10^{-6}$ & 2.4$\times10^{-5}$ & 9.9$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-5}$ & 1.2$\times10^{-5}$ & 1.7$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.3$\times10^{-4}$ & 2.1$\times10^{36}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 30.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 3.2$\times10^{-5}$ & 2.6$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 30.0 & 40.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &8.1$\times10^{-6}$ & 2.5$\times10^{-5}$ & 1.0$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.5$\times10^{-5}$ & 1.3$\times10^{-5}$ & 1.9$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 50.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-7}$ & 1.2$\times10^{-4}$ & 2.1$\times10^{36}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 50.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-6}$ & 3.2$\times10^{-5}$ & 2.5$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.5$\times10^{-6}$ & 2.6$\times10^{-5}$ & 1.1$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 50.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.6$\times10^{-5}$ & 1.4$\times10^{-5}$ & 2.0$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 70.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 1.3$\times10^{-4}$ & 2.2$\times10^{36}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 70.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-6}$ & 3.5$\times10^{-5}$ & 2.8$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.8$\times10^{-6}$ & 2.7$\times10^{-5}$ & 1.1$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-5}$ & 1.5$\times10^{-5}$ & 2.1$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 90.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.7$\times10^{-7}$ & 1.3$\times10^{-4}$ & 2.2$\times10^{36}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 90.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-6}$ & 3.6$\times10^{-5}$ & 2.9$\times10^{37}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 90.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &9.2$\times10^{-6}$ & 2.8$\times10^{-5}$ & 1.2$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.94 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-5}$ & 1.6$\times10^{-5}$ & 2.3$\times10^{38}$ & 2.5$\times10^{-3}$\\
S & -0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-7}$ & 2.3$\times10^{-4}$ & 1.9$\times10^{35}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 10.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 3.7$\times10^{-5}$ & 2.1$\times10^{36}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 10.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &6.9$\times10^{-6}$ & 2.8$\times10^{-5}$ & 1.2$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-5}$ & 1.3$\times10^{-5}$ & 1.9$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 2.2$\times10^{-4}$ & 1.8$\times10^{35}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 30.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 3.5$\times10^{-5}$ & 2.0$\times10^{36}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Pass &6.9$\times10^{-6}$ & 2.9$\times10^{-5}$ & 1.2$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-5}$ & 1.3$\times10^{-5}$ & 1.9$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 50.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &9.8$\times10^{-8}$ & 2.1$\times10^{-4}$ & 1.7$\times10^{35}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 50.0 & 10.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-6}$ & 3.5$\times10^{-5}$ & 2.0$\times10^{36}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 50.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &6.6$\times10^{-6}$ & 2.7$\times10^{-5}$ & 1.1$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass &1.1$\times10^{-5}$ & 1.2$\times10^{-5}$ & 1.9$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 70.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &10.0$\times10^{-8}$ & 2.1$\times10^{-4}$ & 1.8$\times10^{35}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 70.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-6}$ & 3.7$\times10^{-5}$ & 2.1$\times10^{36}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 70.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &6.4$\times10^{-6}$ & 2.6$\times10^{-5}$ & 1.1$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-5}$ & 1.2$\times10^{-5}$ & 1.9$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.0$\times10^{-7}$ & 2.2$\times10^{-4}$ & 1.8$\times10^{35}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 90.0 & 10.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-6}$ & 4.0$\times10^{-5}$ & 2.3$\times10^{36}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 90.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail &6.4$\times10^{-6}$ & 2.6$\times10^{-5}$ & 1.1$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & -0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &1.1$\times10^{-5}$ & 1.2$\times10^{-5}$ & 1.9$\times10^{37}$ & 3.5$\times10^{-4}$\\
S & 0.0 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &5.8$\times10^{-8}$ & 4.5$\times10^{-4}$ & 1.2$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 10.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.1$\times10^{-7}$ & 6.6$\times10^{-5}$ & 1.1$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 10.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.7$\times10^{-6}$ & 3.9$\times10^{-5}$ & 5.6$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail &4.6$\times10^{-6}$ & 1.7$\times10^{-5}$ & 8.9$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-8}$ & 4.3$\times10^{-4}$ & 1.1$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 30.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &4.8$\times10^{-7}$ & 6.3$\times10^{-5}$ & 9.9$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 30.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-6}$ & 3.8$\times10^{-5}$ & 5.4$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 30.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.3$\times10^{-6}$ & 1.6$\times10^{-5}$ & 8.4$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.3$\times10^{-8}$ & 4.2$\times10^{-4}$ & 1.1$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 50.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-7}$ & 6.1$\times10^{-5}$ & 9.7$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 50.0 & 40.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.7$\times10^{-6}$ & 4.0$\times10^{-5}$ & 5.7$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.7$\times10^{-6}$ & 1.7$\times10^{-5}$ & 9.3$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 70.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &5.3$\times10^{-8}$ & 4.2$\times10^{-4}$ & 1.1$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 70.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-7}$ & 6.5$\times10^{-5}$ & 1.0$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 70.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-6}$ & 4.1$\times10^{-5}$ & 5.9$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &4.8$\times10^{-6}$ & 1.8$\times10^{-5}$ & 9.7$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &5.3$\times10^{-8}$ & 4.2$\times10^{-4}$ & 1.1$\times10^{35}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 90.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &5.2$\times10^{-7}$ & 6.8$\times10^{-5}$ & 1.1$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 90.0 & 40.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-6}$ & 4.0$\times10^{-5}$ & 5.9$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.0 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &4.9$\times10^{-6}$ & 1.8$\times10^{-5}$ & 9.9$\times10^{36}$ & 4.0$\times10^{-4}$\\
S & 0.5 & 10.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.6$\times10^{-8}$ & 1.1$\times10^{-3}$ & 1.1$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.1$\times10^{-7}$ & 1.6$\times10^{-4}$ & 8.9$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 10.0 & 40.0 & Fail & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.5$\times10^{-6}$ & 9.8$\times10^{-5}$ & 9.5$\times10^{36}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &5.7$\times10^{-6}$ & 3.7$\times10^{-5}$ & 2.2$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 30.0 & 1.0 & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass &2.5$\times10^{-8}$ & 1.1$\times10^{-3}$ & 1.1$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 30.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.0$\times10^{-7}$ & 1.5$\times10^{-4}$ & 8.4$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 30.0 & 40.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.7$\times10^{-6}$ & 1.1$\times10^{-4}$ & 1.0$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &5.7$\times10^{-6}$ & 3.9$\times10^{-5}$ & 2.3$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 50.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.4$\times10^{-8}$ & 1.1$\times10^{-3}$ & 1.0$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 50.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.9$\times10^{-7}$ & 1.5$\times10^{-4}$ & 8.2$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 50.0 & 40.0 & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.9$\times10^{-6}$ & 1.2$\times10^{-4}$ & 1.1$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-6}$ & 4.2$\times10^{-5}$ & 2.5$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 70.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.4$\times10^{-8}$ & 1.0$\times10^{-3}$ & 1.0$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 70.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.0$\times10^{-7}$ & 1.5$\times10^{-4}$ & 8.6$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 70.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.0$\times10^{-6}$ & 1.3$\times10^{-4}$ & 1.2$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 70.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-6}$ & 4.1$\times10^{-5}$ & 2.5$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 90.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 1.0$\times10^{-3}$ & 9.9$\times10^{34}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 90.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &2.2$\times10^{-7}$ & 1.7$\times10^{-4}$ & 9.4$\times10^{35}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 90.0 & 40.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &2.9$\times10^{-6}$ & 1.2$\times10^{-4}$ & 1.2$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.5 & 90.0 & 160.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.1$\times10^{-6}$ & 4.0$\times10^{-5}$ & 2.4$\times10^{37}$ & 8.4$\times10^{-4}$\\
S & 0.94 & 10.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass &8.8$\times10^{-9}$ & 8.0$\times10^{-3}$ & 2.0$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.7$\times10^{-8}$ & 1.7$\times10^{-3}$ & 1.0$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.4$\times10^{-7}$ & 9.7$\times10^{-4}$ & 6.9$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &6.9$\times10^{-7}$ & 3.7$\times10^{-4}$ & 1.4$\times10^{38}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 30.0 & 1.0 & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &8.3$\times10^{-9}$ & 7.5$\times10^{-3}$ & 1.9$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 30.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.4$\times10^{-8}$ & 1.6$\times10^{-3}$ & 9.7$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 30.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.5$\times10^{-7}$ & 1.0$\times10^{-3}$ & 7.2$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 30.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &7.0$\times10^{-7}$ & 3.7$\times10^{-4}$ & 1.4$\times10^{38}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 50.0 & 1.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &7.7$\times10^{-9}$ & 7.0$\times10^{-3}$ & 1.7$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 50.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 1.5$\times10^{-3}$ & 8.7$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 50.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass &3.7$\times10^{-7}$ & 1.0$\times10^{-3}$ & 7.5$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 50.0 & 160.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &7.9$\times10^{-7}$ & 4.2$\times10^{-4}$ & 1.6$\times10^{38}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 70.0 & 1.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Pass &7.5$\times10^{-9}$ & 6.8$\times10^{-3}$ & 1.7$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 70.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Fail & Fail & Pass &3.9$\times10^{-8}$ & 1.5$\times10^{-3}$ & 8.6$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 70.0 & 40.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Pass &3.8$\times10^{-7}$ & 1.1$\times10^{-3}$ & 7.8$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 70.0 & 160.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.5$\times10^{-7}$ & 4.4$\times10^{-4}$ & 1.7$\times10^{38}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 90.0 & 1.0 & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &7.4$\times10^{-9}$ & 6.6$\times10^{-3}$ & 1.7$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 90.0 & 10.0 & Fail & Fail & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Pass &4.1$\times10^{-8}$ & 1.5$\times10^{-3}$ & 9.0$\times10^{36}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 90.0 & 40.0 & Fail & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Pass &3.9$\times10^{-7}$ & 1.1$\times10^{-3}$ & 7.9$\times10^{37}$ & 4.3$\times10^{-2}$\\
S & 0.94 & 90.0 & 160.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass &8.6$\times10^{-7}$ & 4.5$\times10^{-4}$ & 1.7$\times10^{38}$ & 4.3$\times10^{-2}$\\
M & -0.94 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.5$\times10^{-8}$ & 1.4$\times10^{-2}$ & 1.1$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &8.9$\times10^{-8}$ & 4.6$\times10^{-3}$ & 1.8$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 1.9$\times10^{-3}$ & 2.6$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-7}$ & 6.9$\times10^{-4}$ & 4.3$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.3$\times10^{-8}$ & 1.4$\times10^{-2}$ & 1.1$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &8.5$\times10^{-8}$ & 4.5$\times10^{-3}$ & 1.7$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.2$\times10^{-7}$ & 1.8$\times10^{-3}$ & 2.4$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.1$\times10^{-7}$ & 6.7$\times10^{-4}$ & 4.1$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.0$\times10^{-8}$ & 1.3$\times10^{-2}$ & 9.9$\times10^{37}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 10.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.8$\times10^{-8}$ & 4.1$\times10^{-3}$ & 1.5$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.1$\times10^{-7}$ & 1.7$\times10^{-3}$ & 2.3$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.9$\times10^{-7}$ & 6.2$\times10^{-4}$ & 3.8$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.6$\times10^{-8}$ & 1.1$\times10^{-2}$ & 9.1$\times10^{37}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &7.1$\times10^{-8}$ & 3.7$\times10^{-3}$ & 1.4$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 1.5$\times10^{-3}$ & 2.1$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.8$\times10^{-7}$ & 5.6$\times10^{-4}$ & 3.5$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.4$\times10^{-8}$ & 1.1$\times10^{-2}$ & 8.6$\times10^{37}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &6.7$\times10^{-8}$ & 3.5$\times10^{-3}$ & 1.3$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &10.0$\times10^{-8}$ & 1.5$\times10^{-3}$ & 2.0$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.7$\times10^{-7}$ & 5.4$\times10^{-4}$ & 3.3$\times10^{38}$ & 3.8$\times10^{-1}$\\
M & -0.5 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.2$\times10^{-8}$ & 4.9$\times10^{-3}$ & 2.7$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.0$\times10^{-8}$ & 2.5$\times10^{-3}$ & 4.6$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 1.4$\times10^{-3}$ & 6.7$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-7}$ & 6.6$\times10^{-4}$ & 1.1$\times10^{38}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.1$\times10^{-8}$ & 4.8$\times10^{-3}$ & 2.7$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &6.7$\times10^{-8}$ & 2.4$\times10^{-3}$ & 4.4$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.9$\times10^{-8}$ & 1.4$\times10^{-3}$ & 6.4$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-7}$ & 6.4$\times10^{-4}$ & 1.1$\times10^{38}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.9$\times10^{-8}$ & 4.5$\times10^{-3}$ & 2.5$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.2$\times10^{-8}$ & 2.2$\times10^{-3}$ & 4.1$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &9.2$\times10^{-8}$ & 1.3$\times10^{-3}$ & 6.0$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-7}$ & 6.0$\times10^{-4}$ & 9.9$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 70.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.6$\times10^{-8}$ & 4.2$\times10^{-3}$ & 2.4$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.7$\times10^{-8}$ & 2.0$\times10^{-3}$ & 3.7$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.5$\times10^{-8}$ & 1.2$\times10^{-3}$ & 5.6$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 5.6$\times10^{-4}$ & 9.2$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.4$\times10^{-8}$ & 3.9$\times10^{-3}$ & 2.2$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-8}$ & 1.9$\times10^{-3}$ & 3.5$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &8.1$\times10^{-8}$ & 1.1$\times10^{-3}$ & 5.3$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 90.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-7}$ & 5.3$\times10^{-4}$ & 8.8$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & 0.0 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.1$\times10^{-8}$ & 5.5$\times10^{-3}$ & 3.7$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 10.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.4$\times10^{-8}$ & 2.7$\times10^{-3}$ & 6.3$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 40.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &8.1$\times10^{-8}$ & 1.7$\times10^{-3}$ & 9.5$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 10.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.3$\times10^{-7}$ & 8.5$\times10^{-4}$ & 1.5$\times10^{37}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &3.1$\times10^{-8}$ & 5.4$\times10^{-3}$ & 3.6$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 10.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &5.2$\times10^{-8}$ & 2.7$\times10^{-3}$ & 6.2$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &7.8$\times10^{-8}$ & 1.6$\times10^{-3}$ & 9.2$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.2$\times10^{-7}$ & 8.2$\times10^{-4}$ & 1.4$\times10^{37}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &3.0$\times10^{-8}$ & 5.2$\times10^{-3}$ & 3.5$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &4.8$\times10^{-8}$ & 2.5$\times10^{-3}$ & 5.7$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &7.3$\times10^{-8}$ & 1.5$\times10^{-3}$ & 8.6$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 7.6$\times10^{-4}$ & 1.3$\times10^{37}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.9$\times10^{-8}$ & 5.0$\times10^{-3}$ & 3.4$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &4.6$\times10^{-8}$ & 2.3$\times10^{-3}$ & 5.4$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.7$\times10^{-8}$ & 1.4$\times10^{-3}$ & 7.9$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 7.0$\times10^{-4}$ & 1.2$\times10^{37}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.6$\times10^{-8}$ & 4.5$\times10^{-3}$ & 3.1$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &4.3$\times10^{-8}$ & 2.2$\times10^{-3}$ & 5.1$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Pass & Fail & Fail & Fail &6.3$\times10^{-8}$ & 1.3$\times10^{-3}$ & 7.4$\times10^{36}$ & 2.3$\times10^{-2}$\\
M & 0.0 & 90.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.0$\times10^{-7}$ & 6.8$\times10^{-4}$ & 1.2$\times10^{37}$ & 2.3$\times10^{-2}$\\
M & 0.5 & 10.0 & 1.0 & Fail & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.4$\times10^{-8}$ & 9.6$\times10^{-3}$ & 3.0$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 10.0 & 10.0 & Pass & Fail & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &4.0$\times10^{-8}$ & 4.6$\times10^{-3}$ & 5.2$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 10.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &6.5$\times10^{-8}$ & 2.7$\times10^{-3}$ & 8.3$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.1$\times10^{-7}$ & 1.3$\times10^{-3}$ & 1.4$\times10^{38}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 30.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &2.3$\times10^{-8}$ & 9.3$\times10^{-3}$ & 2.9$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 30.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.9$\times10^{-8}$ & 4.4$\times10^{-3}$ & 5.0$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 30.0 & 40.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &6.3$\times10^{-8}$ & 2.6$\times10^{-3}$ & 8.0$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &1.0$\times10^{-7}$ & 1.3$\times10^{-3}$ & 1.3$\times10^{38}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 50.0 & 1.0 & Fail & Fail & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &2.2$\times10^{-8}$ & 9.0$\times10^{-3}$ & 2.8$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 50.0 & 10.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &3.7$\times10^{-8}$ & 4.2$\times10^{-3}$ & 4.8$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 50.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail &6.0$\times10^{-8}$ & 2.5$\times10^{-3}$ & 7.7$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 50.0 & 160.0 & Pass & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.0$\times10^{-7}$ & 1.2$\times10^{-3}$ & 1.3$\times10^{38}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 70.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &2.1$\times10^{-8}$ & 8.7$\times10^{-3}$ & 2.7$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.5$\times10^{-8}$ & 4.0$\times10^{-3}$ & 4.5$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 70.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 2.3$\times10^{-3}$ & 7.1$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 70.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.6$\times10^{-8}$ & 1.2$\times10^{-3}$ & 1.2$\times10^{38}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 90.0 & 1.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.0$\times10^{-8}$ & 7.9$\times10^{-3}$ & 2.5$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 90.0 & 10.0 & Pass & Fail & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.3$\times10^{-8}$ & 3.8$\times10^{-3}$ & 4.2$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 90.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 2.3$\times10^{-3}$ & 6.9$\times10^{37}$ & 2.5$\times10^{-1}$\\
M & 0.5 & 90.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &9.3$\times10^{-8}$ & 1.1$\times10^{-3}$ & 1.2$\times10^{38}$ & 2.5$\times10^{-1}$\\
M & 0.94 & 10.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail &1.7$\times10^{-8}$ & 7.4$\times10^{-2}$ & 1.4$\times10^{38}$ & 1.6\\
M & 0.94 & 10.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.5$\times10^{-8}$ & 2.0$\times10^{-2}$ & 2.0$\times10^{38}$ & 1.6\\
M & 0.94 & 10.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.6$\times10^{-8}$ & 8.5$\times10^{-3}$ & 3.0$\times10^{38}$ & 1.6\\
M & 0.94 & 10.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &5.8$\times10^{-8}$ & 3.1$\times10^{-3}$ & 4.8$\times10^{38}$ & 1.6\\
M & 0.94 & 30.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Fail & Pass & Pass & Pass & Fail & Fail & Fail &1.6$\times10^{-8}$ & 7.1$\times10^{-2}$ & 1.3$\times10^{38}$ & 1.6\\
M & 0.94 & 30.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &2.4$\times10^{-8}$ & 2.0$\times10^{-2}$ & 2.0$\times10^{38}$ & 1.6\\
M & 0.94 & 30.0 & 40.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &3.5$\times10^{-8}$ & 8.2$\times10^{-3}$ & 2.9$\times10^{38}$ & 1.6\\
M & 0.94 & 30.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail &5.7$\times10^{-8}$ & 3.0$\times10^{-3}$ & 4.7$\times10^{38}$ & 1.6\\
M & 0.94 & 50.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail &1.6$\times10^{-8}$ & 6.8$\times10^{-2}$ & 1.3$\times10^{38}$ & 1.6\\
M & 0.94 & 50.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-8}$ & 1.9$\times10^{-2}$ & 1.9$\times10^{38}$ & 1.6\\
M & 0.94 & 50.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &3.4$\times10^{-8}$ & 7.9$\times10^{-3}$ & 2.8$\times10^{38}$ & 1.6\\
M & 0.94 & 50.0 & 160.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &5.5$\times10^{-8}$ & 2.9$\times10^{-3}$ & 4.5$\times10^{38}$ & 1.6\\
M & 0.94 & 70.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.5$\times10^{-8}$ & 6.4$\times10^{-2}$ & 1.2$\times10^{38}$ & 1.6\\
M & 0.94 & 70.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-8}$ & 1.8$\times10^{-2}$ & 1.8$\times10^{38}$ & 1.6\\
M & 0.94 & 70.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &3.2$\times10^{-8}$ & 7.6$\times10^{-3}$ & 2.7$\times10^{38}$ & 1.6\\
M & 0.94 & 70.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.5$\times10^{-8}$ & 2.9$\times10^{-3}$ & 4.5$\times10^{38}$ & 1.6\\
M & 0.94 & 90.0 & 1.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.4$\times10^{-8}$ & 6.1$\times10^{-2}$ & 1.2$\times10^{38}$ & 1.6\\
M & 0.94 & 90.0 & 10.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &2.0$\times10^{-8}$ & 1.7$\times10^{-2}$ & 1.7$\times10^{38}$ & 1.6\\
M & 0.94 & 90.0 & 40.0 & Pass & Pass & Fail & Fail & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &3.1$\times10^{-8}$ & 7.2$\times10^{-3}$ & 2.5$\times10^{38}$ & 1.6\\
M & 0.94 & 90.0 & 160.0 & Pass & Pass & Fail & Pass & Fail & Pass & Fail & Pass & Fail & Fail & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 2.8$\times10^{-3}$ & 4.4$\times10^{38}$ & 1.6\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Koral_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{cccc|ccc|c|cccccc|c|c|c|cccc}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Koral Thermal Models}
\label{tab:koralPF}
\tablehead{ \colhead{M/S}  &  %
\colhead{Spin}  &  %
\colhead{$i$}  &  %
\colhead{$\Rh$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
\colhead{$\dot{M}/\dot{M}_{Edd}$}  &  %
\colhead{$P_{out}$(cgs)}  &  %
\colhead{$P_{out}/(\dot{M} c^2)$}}
\startdata
M & -0.9 & 10.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.9$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.9 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.8$\times10^{-8}$ & 2.7$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.9 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.6$\times10^{-8}$ & 2.5$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.9 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.3$\times10^{-8}$ & 2.3$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.9 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &2.2$\times10^{-8}$ & 2.2$\times10^{37}$ & 1.9$\times10^{-1}$\\
M & -0.7 & 10.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-8}$ & 3.2$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.7 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-8}$ & 3.0$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.7 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.3$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.7 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.9$\times10^{-8}$ & 2.5$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.7 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &3.8$\times10^{-8}$ & 2.5$\times10^{37}$ & 1.3$\times10^{-1}$\\
M & -0.5 & 10.0 & 20.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.5$\times10^{-8}$ & 3.5$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.2$\times10^{-8}$ & 3.3$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.8$\times10^{-8}$ & 3.1$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.3$\times10^{-8}$ & 2.8$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.5 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.9$\times10^{-8}$ & 2.6$\times10^{37}$ & 1.0$\times10^{-1}$\\
M & -0.3 & 10.0 & 20.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.5$\times10^{-8}$ & 2.8$\times10^{37}$ & 7.2$\times10^{-2}$\\
M & -0.3 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.2$\times10^{-8}$ & 2.7$\times10^{37}$ & 7.2$\times10^{-2}$\\
M & -0.3 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.7$\times10^{-8}$ & 2.5$\times10^{37}$ & 7.2$\times10^{-2}$\\
M & -0.3 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.1$\times10^{-8}$ & 2.2$\times10^{37}$ & 7.2$\times10^{-2}$\\
M & -0.3 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.8$\times10^{-8}$ & 2.1$\times10^{37}$ & 7.2$\times10^{-2}$\\
M & 0.0 & 10.0 & 20.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.9$\times10^{-8}$ & 1.4$\times10^{37}$ & 3.4$\times10^{-2}$\\
M & 0.0 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.7$\times10^{-8}$ & 1.4$\times10^{37}$ & 3.4$\times10^{-2}$\\
M & 0.0 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &7.3$\times10^{-8}$ & 1.3$\times10^{37}$ & 3.4$\times10^{-2}$\\
M & 0.0 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.7$\times10^{-8}$ & 1.2$\times10^{37}$ & 3.4$\times10^{-2}$\\
M & 0.0 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &6.3$\times10^{-8}$ & 1.1$\times10^{37}$ & 3.4$\times10^{-2}$\\
M & 0.3 & 10.0 & 20.0 & Pass & Fail & Pass & Fail & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.7$\times10^{-8}$ & 4.2$\times10^{37}$ & 1.4$\times10^{-1}$\\
M & 0.3 & 30.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &5.6$\times10^{-8}$ & 4.1$\times10^{37}$ & 1.4$\times10^{-1}$\\
M & 0.3 & 50.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.4$\times10^{-8}$ & 3.9$\times10^{37}$ & 1.4$\times10^{-1}$\\
M & 0.3 & 70.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &5.0$\times10^{-8}$ & 3.6$\times10^{37}$ & 1.4$\times10^{-1}$\\
M & 0.3 & 90.0 & 20.0 & Pass & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Pass & Fail & Fail & Fail & Fail &4.7$\times10^{-8}$ & 3.4$\times10^{37}$ & 1.4$\times10^{-1}$\\
M & 0.9 & 10.0 & 20.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail &1.4$\times10^{-8}$ & 9.5$\times10^{37}$ & 1.3\\
M & 0.9 & 30.0 & 20.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Fail & Fail & Fail & Fail &1.4$\times10^{-8}$ & 9.1$\times10^{37}$ & 1.3\\
M & 0.9 & 50.0 & 20.0 & Pass & Pass & Fail & Fail & Pass & Pass & Pass & Pass & Pass & Fail & Fail & Fail & Fail &1.3$\times10^{-8}$ & 8.6$\times10^{37}$ & 1.3\\
M & 0.9 & 70.0 & 20.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.2$\times10^{-8}$ & 8.0$\times10^{37}$ & 1.3\\
M & 0.9 & 90.0 & 20.0 & Pass & Fail & Fail & Fail & Pass & Pass & Pass & Fail & Fail & Fail & Fail & Fail & Fail &1.1$\times10^{-8}$ & 7.6$\times10^{37}$ & 1.3\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/Ressler_Table.tex <==
\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{c|ccc|c|cccccc|c|c|c}
\tabletypesize{\scriptsize}
\tablecaption{Pass/Fail Table, Wind Fed Models}
\label{tab:resslerPF}
\tablehead{ \colhead{$\beta$}  &  %
\colhead{$F_{86}$}  &  %
\colhead{$\lambda_{maj,86}$}  &  %
\colhead{$F_{2\mu{\rm m}}$}  &  %
\colhead{non-EHT}  &  %
\colhead{$\lambda_{230}$}  &  %
\colhead{Nulls}  &  %
\colhead{Ring D}  &  %
\colhead{Ring W}  &  %
\colhead{Ring A}  &  %
\colhead{4G$\lambda$} & %
\colhead{EHT}  &  %
\colhead{All}  &  %
\colhead{M$_3$} & %
}
\startdata
1E2 & Fail & Pass & Fail & Fail & Pass & Pass & Pass & Fail & Pass & Pass & Fail & Fail & Fail\\
1E6 & Fail & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Pass & Pass & Fail & Fail & Fail\\
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Tables/fail_one.tex <==
\begin{deluxetable*}{l|ccccc}\label{tab:fail_one}
\tablecaption{Models that fail only one constraint}
\tablehead{
\colhead{Code/Setup} &
\colhead{MAD/SANE} &
\colhead{spin} &
\colhead{inc} &
\colhead{$\Rh$} &
\colhead{Constraint Failed}
}
\startdata
\kharma Thermal					&	SANE	&	0.94	&	10		&	40		&	86\,GHz size		\\
\kharma Thermal					&	SANE	&	0.94	&	30		&	40		&	86\,GHz size		\\
\kharma Thermal					&	SANE	&	0.94	&	50		&	1		&	86\,GHz size		\\
\kharma Thermal					&	MAD		&	0.5		&	30		&	40		&	\mi{3}				\\
\kharma Thermal					&	MAD		&	0.5		&	30		&	160		&	\mi{3}				\\
\kharma Thermal					&	MAD		&	0.94	&	10		&	160		&	\mi{3}				\\
\kharma Thermal					&	MAD		&	0.94	&	30		&	160		&	\mi{3}				\\
\hline
\bhac Thermal					&	SANE	&	-0.5	&	30		&	40		&	Mring diameter   	\\
\bhac Thermal					&	SANE	&	0		&	30		&	40		&	Mring diameter   	\\
\bhac Thermal					&	SANE	&	0.5		&	10		&	40		&   \mi{3}  			\\
\bhac Thermal					&	SANE	&	0.5		&	10		&	160		&   \mi{3}  			\\
\bhac Thermal					&	SANE	&	0.5		&	30		&	40		&   \mi{3}  			\\
\bhac Thermal					&	SANE	&	0.5		&	30		&	160		&   \mi{3}  			\\
\bhac Thermal					&	MAD		&	0.5		&	30		&	160		&   \mi{3}  			\\
\bhac Thermal					&	MAD		&	0.5		&	50		&	160		&   \mi{3}  			\\
\bhac Thermal					&	MAD		&	0.94	&	10		&	160		&   \mi{3}  			\\
\bhac Thermal					&	MAD		&	0.94	&	30		&	160		&   \mi{3}  			\\
\hline
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0		&	70		&	1		&	86\,GHz flux		\\	  
\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	10		&	40		&	2.2\,$\mu$m flux	\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	10		&	40		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	10		&	80		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	10		&	160		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	30		&	40		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	30		&	80		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	SANE	&	0.5		&	30		&	160		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	30		&	80		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	50		&	160		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.94	&	10		&	160		&	\mi{3}   			\\	  
\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	30		&	160		&	\mi{3}				\\	  
%\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	10		&	80		&	??					\\	%This fail two constraints, but only in the extended 15kM runs  
%\bhac $\kappa(\sigma, \beta)$	&	MAD		&	0.5		&	10		&	160		&	??					\\	%This fail two constraints, but only in the extended 15kM runs   
\hline
\bhac $\epsilon = 0.05$			&	SANE	&	0.94	&	10		&	10		&	\mi{3}   			\\	
\bhac $\epsilon = 0.05$			&	SANE	&	0.94	&	30		&	10		&	86\,GHz flux   		\\	
\bhac $\epsilon = 0.05$			&	MAD		&	0.5		&	30		&	160		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.05$			&	MAD		&	0.5		&	50		&	160		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.05$			&	MAD		&	0.94	&	10		&	40		&	2.2\,$\mu$m flux   	\\	
\hline
\bhac $\epsilon = 0.10$			&	SANE	&	0.94	&	10		&	10		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.10$			&	MAD		&	0.5		&	30		&	160		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.10$			&	MAD		&	0.5		&	50		&	160		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.10$			&	MAD		&	0.94	&	10		&	40		&	2.2\,$\mu$m flux   	\\	
\hline
\bhac $\epsilon = 0.20$			&	SANE	&	0.94	&	10		&	10		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.20$			&	MAD		&	0.94	&	10		&	40		&	2.2\,$\mu$m flux   	\\	
\bhac $\epsilon = 0.20$			&	MAD		&	0.94	&	10		&	160		&	2.2\,$\mu$m flux   	\\	
\hline
\bhac $\kappa = 5$				&	MAD		&	0.94	&	50		&	1		&	2.2\,$\mu$m flux   	\\	
\hline
\hamr 30$^\circ$ tilt  			&	INSANE	&	0.94	&	10		&	160		&	86\,GHz size		\\	
\enddata
\tablecomments{Models which pass all of the constraints except for one. Since no model passes all constraints, these represent the parameters that are closest to being consistent with observations.}

\end{deluxetable*}

